A Simple and Adaptive Learning Rate for FTRL in Online Learning with Minimax Regret of $\Theta(T^{2/3})$ and its Application to Best-of-Both-Worlds

Follow-the-Regularized-Leader (FTRL) is a powerful framework for various online learning problems. By designing its regularizer and learning rate to be adaptive to past observations, FTRL is known to work adaptively to various properties of an underlying environment. However, most existing adaptive learning rates are for online learning problems with a minimax regret of $\Theta(\sqrt{T})$ for the number of rounds $T$, and there are only a few studies on adaptive learning rates for problems with a minimax regret of $\Theta(T^{2/3})$, which include several important problems dealing with indirect feedback. To address this limitation, we establish a new adaptive learning rate framework for problems with a minimax regret of $\Theta(T^{2/3})$. Our learning rate is designed by matching the stability, penalty, and bias terms that naturally appear in regret upper bounds for problems with a minimax regret of $\Theta(T^{2/3})$. As applications of this framework, we consider three major problems with a minimax regret of $\Theta(T^{2/3})$: partial monitoring, graph bandits, and multi-armed bandits with paid observations. We show that FTRL with our learning rate and the Tsallis entropy regularizer improves existing Best-of-Both-Worlds (BOBW) regret upper bounds, which achieve simultaneous optimality in the stochastic and adversarial regimes. The resulting learning rate is surprisingly simple compared to the existing learning rates for BOBW algorithms for problems with a minimax regret of $\Theta(T^{2/3})$.

==> tex_src/app_notation.tex <==
\section{Notation}\label{app:notation}

Table~\ref{table:notation} summarizes the symbols used in this paper.

% =======================
\begin{table}[h]
  \caption{
  Notation
  }
  \label{table:notation}
  \centering
%  \footnotesize
  \begin{tabular}{ll}
    \toprule
    Symbol & Meaning  \\
    \midrule
    $\calP_k$ & $(k-1)$-dimensional probability simplex \\
    $T \in \N$ & time horizon \\
    $k \in \N$ & number of arms (or actions) \\
    $A_t \in [k]$ & arm (or action) chosen by learner at round $t$  \\
    \midrule
%    $a^* \in [k]$ & optimal arm \\
    $s \leq k$ & $\max_t \nrm{\ell_t}_0$, sparsity level of losses \\
    $L_2$ & $\sumT \nrm{\ell_t}^2$ \\
    \midrule
    $\lossmat \in [0,1]^{k \times d}$ & loss matrix  \\ 
    $\Sigma$ & set of feedback symbols  \\ 
    $\fbmat \in \Sigma^{k \times d}$ & feedback matrix  \\ 
    $d \in \N$ & number of outcomes  \\ 
    $m \in \N$ & maximum number of distinct symbols in a single row of $\Phi$ \\ 
    $x_t \in [d]$ & outcome chosen by opponent at round $t$  \\
    \midrule
    $q_t \in \calP_k$ & output of FTRL at round $t$   \\ 
    $p_t \in \calP_k$ & arm selection probability at round $t$   \\ 
    $\Phi_t \colon \calP_k \to \R$ & regularizer of FTRL at round $t$  \\ 
    $\eta_t = 1/\beta_t > 0$  & learning rate of FTRL at round $t$ \\ 
    $\psiNS \colon \R_+^k \to \R $ & $\sumk x_i \log x_i $, negative Shannon entropy  \\ 
    $\psiLB \colon \R_+^k \to \R $ & $\sumk \log(1/x_i) $, log-barrier \\ 
    $\phiNS \colon \R_+ \to \R$ & $x \log x  $  \\ 
    $\phiLB  \colon \R_+ \to \R$ & $\log(1/x) $  \\ 
    \midrule 
    $h_t$ &  penalty component at round $t$ \\
    $\zF_t$ &  stability component at round $t$ \\
%    $\zmax_t$ & (basically) an upper bound of stability component at round $t$ \\
    \midrule
    $\omega_t$   &  stability component  $\zF_t$ introduced in~\eqref{eq:def_eta_sparse_and_omega} (Section~\ref{subsec:sparse_std}) \\
    $\nu_t$   &  stability component $\zF_t$ introduced in~\eqref{eq:def_eta_sparse_negative_losses_and_nu} (Section~\ref{subsec:sparse_negtive_losse}) \\
    $V'_t$   &  stability component $\zF_t$ introduced in~\eqref{eq:def_eta_pm} (Appendix~\ref{app:pm_detailed}) \\
    \midrule
    $C \geq 0 $ & corruption level \\
    \bottomrule
  \end{tabular}
\end{table}
% =======================




